Scribble2Label: Scribble-Supervised Cell Segmentation via Self-Generating Pseudo-Labels with Consistency

Segmentation is a fundamental process in microscopic cell image analysis. With the advent of recent advances in deep learning, more accurate and high-throughput cell segmentation has become feasible. However, most existing deep learning-based cell segmentation algorithms require fully annotated ground-truth cell labels, which are time-consuming and labor-intensive to generate. In this paper, we introduce Scribble2Label, a novel weakly-supervised cell segmentation framework that exploits only a handful of scribble annotations without full segmentation labels. The core idea is to combine pseudo-labeling and label filtering to generate reliable labels from weak supervision. For this, we leverage the consistency of predictions by iteratively averaging the predictions to improve pseudo labels. We demonstrate the performance of Scribble2Label by comparing it to several state-of-the-art cell segmentation methods with various cell image modalities, including bright-field, fluorescence, and electron microscopy. We also show that our method performs robustly across different levels of scribble details, which confirms that only a few scribble annotations are required in real-use cases.

==> Related_Work.tex <==
% !TEX root = root.tex

%%%
\begin{figure}[!t]
\centering
\includegraphics[width=1\textwidth]{Generation}
\caption{A self-generated label of a training image during the training. \textcolor{yellow}{Yellow}: scribble for background, \textcolor{blue}{Blue}: scribble for cell, \textcolor{red}{Red}: the pixels below consistency threshold $\uptau$. these pixels are ignored when calculating unscribbled loss. White and Black are the cell or background pixels over $\uptau$. The scores show IoU compared with the ground truth.}
\label{fig_generation}
\end{figure}
%%%
\subsection{Cell Segmentation}
Cell segmentation is an important step in cell imaging analysis and has been steadily being studied in the field of computer vision. Methods vary: Segmentation based on Watershed \cite{yang2006nuclei}, Chan-vese with edge model \cite{mavska2013segmentation} and gradient vector flow \cite{li2005segmentation}.
Since the introduction of deep learning, the performance of cell segmentation has improved significantly. However, deep learning based cell segmentation methods \cite{xing2015automatic,arbelle2019microscopy,yi2019multi} require a fully annotated label. This is time-consuming to make and can be done by professionals, which is expensive.

\subsection{Weakly-supervised Cell Segmentation}
Recently, weakly-supervised cell segmentation has been studied. Annotating all areas of a cell requires a lot of time and expert knowledge. To solve this problem, cell segmentation was performed using a point annotation. \cite{yoo2019pseudoedgenet, qu2019weakly} used Voronoi Edge to create a new coarse label and used it to segment cells in histopathology images. In \cite{nishimura2019weakly}, the point detection network is trained using point annotation, and the cell instance segmentation is performed by using the image area that affects the backpropagation of the center point of the detected cell.
However, there are still too many nuclei in a cell image. Moreover, the point location affects the performance of point-based methods. Annotating the center of many cells requires concentration. So we propose a scribble-supervised cell segmentation algorithm that learns by simply annotating a small number of cells and backgrounds with a scribble.

\subsection{Scribble-supervised Learning}
Scribble is one of the simple annotation methods. Scribble is widely used in interactive image segmentation\cite{lin2016scribblesup}. Scribble-supervised Learning is a way to train a model with only scribble labels.
Scribble-supervised Learning exploits scribble-label itself and regularized the network with standard segmentation technique or additional parameters\cite{lin2016scribblesup, tang2018regularized, can2018learning, wang2019boundary, wu2018scribble}. \cite{lin2016scribblesup} regularizes the proposal generation by graph-cut. DenseCRF is helpful for scribble-supervised learning for re-labeling\cite{can2018learning} or being integrating as a loss\cite{tang2018regularized}. The additional model parameters are also helpful for improving scribble supervised learning, such as boundary prediction\cite{wang2019boundary} and discriminator\cite{wu2018scribble}.
Unlike previous methods, \texttt{Scribble2Label} doesn't require additional standard segmentation computation or model parameters. The network generates a reliable label from scribble by combining pseudo-labeling and label-filtering. 

\subsection{Semi-supervised Learning}
Semi-supervised Learning (SSL) is a method of training a model using a few labeled data and a large number of unlabeled data. In SSL, entropy minimization generally enforces that the classifier's decision boundary doesn't pass the high-density regions of the marginal data distribution \cite{berthelot2019mixmatch}. Entropy minimization makes output low-entropy prediction from the unlabeled data. \cite{lee2013pseudo, sohn2020fixmatch} utilize pseudo-labeling to make one-hot encoding a sample with high prediction confidence. \cite{berthelot2019mixmatch} makes the sharpen target distribution, which is closer to the one-hot distribution. \cite{hung2018adversarial} uses pseudo-labeling to generate confidence values from discriminators. \texttt{Scribble2Label} suggests a pseudo-labeling method that collaborates with the consistency of prediction.

==> tutorial.tex <==
\section{First Section}
\subsection{A Subsection Sample}
Please note that the first paragraph of a section or subsection is
not indented. The first paragraph that follows a table, figure,
equation etc. does not need an indent, either.

Subsequent paragraphs, however, are indented.

\subsubsection{Sample Heading (Third Level)} Only two levels of
headings should be numbered. Lower level headings remain unnumbered;
they are formatted as run-in headings.

\paragraph{Sample Heading (Fourth Level)}
The contribution should contain no more than four levels of
headings. Table~\ref{tab1} gives a summary of all heading levels.

\begin{table}
\caption{Table captions should be placed above the
tables.}\label{tab1}
\begin{tabular}{|l|l|l|}
\hline
Heading level &  Example & Font size and style\\
\hline
Title (centered) &  {\Large\bfseries Lecture Notes} & 14 point, bold\\
1st-level heading &  {\large\bfseries 1 Introduction} & 12 point, bold\\
2nd-level heading & {\bfseries 2.1 Printing Area} & 10 point, bold\\
3rd-level heading & {\bfseries Run-in Heading in Bold.} Text follows & 10 point, bold\\
4th-level heading & {\itshape Lowest Level Heading.} Text follows & 10 point, italic\\
\hline
\end{tabular}
\end{table}


\noindent Displayed equations are centered and set on a separate
line.
\begin{equation}
x + y = z
\end{equation}
Please try to avoid rasterized images for line-art diagrams and
schemas. Whenever possible, use vector graphics instead (see
Fig.~\ref{fig1}).

\begin{figure}
\includegraphics[width=\textwidth]{fig1.eps}
\caption{A figure caption is always placed below the illustration.
Please note that short captions are centered, while long ones are
justified by the macro package automatically.} \label{fig1}
\end{figure}

\begin{theorem}
This is a sample theorem. The run-in heading is set in bold, while
the following text appears in italics. Definitions, lemmas,
propositions, and corollaries are styled the same way.
\end{theorem}
%
% the environments 'definition', 'lemma', 'proposition', 'corollary',
% 'remark', and 'example' are defined in the LLNCS documentclass as well.
%
\begin{proof}
Proofs, examples, and remarks have the initial word in italics,
while the following text appears in normal font.
\end{proof}
For citations of references, we prefer the use of square brackets
and consecutive numbers. Citations using labels or the author/year
convention are also acceptable. The following bibliography provides
a sample reference list with entries for journal
articles~\cite{ref_article1}, an LNCS chapter~\cite{ref_lncs1}, a
book~\cite{ref_book1}, proceedings without editors~\cite{ref_proc1},
and a homepage~\cite{ref_url1}. Multiple citations are grouped
\cite{ref_article1,ref_lncs1,ref_book1},
\cite{ref_article1,ref_book1,ref_proc1,ref_url1}.

%
\begin{thebibliography}{8}
\bibitem{ref_article1}
Author, F.: Article title. Journal \textbf{2}(5), 99--110 (2016)

\bibitem{ref_lncs1}
Author, F., Author, S.: Title of a proceedings paper. In: Editor,
F., Editor, S. (eds.) CONFERENCE 2016, LNCS, vol. 9999, pp. 1--13.
Springer, Heidelberg (2016). \doi{10.10007/1234567890}

\bibitem{ref_book1}
Author, F., Author, S., Author, T.: Book title. 2nd edn. Publisher,
Location (1999)

\bibitem{ref_proc1}
Author, A.-B.: Contribution title. In: 9th International Proceedings
on Proceedings, pp. 1--2. Publisher, Location (2010)

\bibitem{ref_url1}
LNCS Homepage, \url{http://www.springer.com/lncs}. Last accessed 4
Oct 2017
\end{thebibliography}
